Adversarial Examples Are Not Bugs, They Are Features

Adversarial examples have attracted significant attention in machine learning, but the reasons for their existence and pervasiveness remain unclear. We demonstrate that adversarial examples can be directly attributed to the presence of non-robust features: features derived from patterns in the data distribution that are highly predictive, yet brittle and incomprehensible to humans. After capturing these features within a theoretical framework, we establish their widespread existence in standard datasets. Finally, we present a simple setting where we can rigorously tie the phenomena we observe in practice to a misalignment between the (human-specified) notion of robustness and the inherent geometry of the data.

==> rethinking.tex <==
Our results suggest that there is nothing mysterious about adversarial examples
and adversarial transferability as a phenomenon.
From a machine learning perspective, we are training standard models to be as
accurate as possible.
As a result, these models will exploit the entirety of input features in order
to make their prediction as long as these features are predictive.
The fact that some of these features are imperceptible to humans (non-robust)
does not diminish their value for performing accurate predictions.
Our experiments establish that these features are indeed sufficient to learn a
good classifier.
It should hence not come as a surprise that standard models will rely heavily on
such imperceptible features, thus being vulnerable to adversarial examples.

This intuition establishes adversarial examples as {\em a purely human
phenomenon}.
Should models operate in isolation, faced only with the task at hand there is
nothing wrong with brittle models.

Something about robustness to naturally arising perturbations (snow, rain).


This, in turn, leads us to a new perspective on adversarial examples as a {\em
fundamentally human} phenomenon. While an abundance of data and supervision has
led humans to discover the correct features to use to for classification tasks,
it turns out that adversarial perturbations to which neural networks are
vulnerable are tangible, {\em well-generalizing} features for modern
classification tasks that simply happen to be imperceptible. 

